Deep Probabilistic Feature-metric Tracking

Dense image alignment from RGB-D images remains a critical issue for real-world applications, especially under challenging lighting conditions and in a wide baseline setting. In this paper, we propose a new framework to learn a pixel-wise deep feature map and a deep feature-metric uncertainty map predicted by a Convolutional Neural Network (CNN), which together formulate a deep probabilistic feature-metric residual of the two-view constraint that can be minimised using Gauss-Newton in a coarse-to-fine optimisation framework. Furthermore, our network predicts a deep initial pose for faster and more reliable convergence. The optimisation steps are differentiable and unrolled to train in an end-to-end fashion. Due to its probabilistic essence, our approach can easily couple with other residuals, where we show a combination with ICP. Experimental results demonstrate state-of-the-art performances on the TUM RGB-D dataset and the 3D rigid object tracking dataset. We further demonstrate our method's robustness and convergence qualitatively.

==> Deep Probabilistic Feature-metric Tracking v2/notation-math-defs.tex <==
\usepackage{xifthen}
\usepackage{xparse}
\usepackage{subdepth}
\usepackage{leftidx}
\usepackage{bm}
\usepackage{amsmath}
%%%%%%%%%%%%%%%%%%%%%
%% Paul and Stefan's Math Defs
%% Operators
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\pd}[2]{{\frac{\partial #1}{\partial #2}}}
%\newcommand{\diag}{\mathrm{diag}}

%% Matrix shortcuts
\newcommand{\bbm}{\begin{bmatrix}}
	\newcommand{\ebm}{\end{bmatrix}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%% UTIAS Notation
%%

% Basic bold for letters and symbols
\DeclareMathAlphabet{\mbf}{OT1}{ptm}{b}{n}
\newcommand{\mbs}[1]{{\bm{#1}}}

% helper bold symbols
\newcommand{\mbsbar}[1]{{\overline{\boldsymbol{#1}}}}
\newcommand{\mbshat}[1]{{\hat{\boldsymbol{#1}}}}
\newcommand{\mbstilde}[1]{{\tilde{\boldsymbol{#1}}}}
\newcommand{\mbsvec}[1]{{\underrightarrow{\boldsymbol{#1}}}}
\newcommand{\mbsdel}[1]{{\delta {\boldsymbol{#1}}}}
\newcommand{\mbsDel}[1]{{\delta {\boldsymbol{#1}}}}
\newcommand{\mbsdot}[1]{{\dot {\boldsymbol{#1}}}}
\newcommand{\mbsddot}[1]{{\ddot {\boldsymbol{#1}}}}
\newcommand{\mbc}[1]{{{\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcbar}[1]{{\overline{\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbchat}[1]{{\hat{\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcvec}[1]{{\underrightarrow{\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcdel}[1]{{\delta {\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcDel}[1]{{\delta {\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcdot}[1]{{\dot {\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbcddot}[1]{{\ddot {\boldsymbol{\mathcal{#1}}}}}
\newcommand{\mbfbar}[1]{{\overline{\mbf{#1}}}}
\newcommand{\mbfhat}[1]{{\hat{\mbf{#1}}}}
\newcommand{\mbftilde}[1]{{\tilde{\mbf{#1}}}}
\newcommand{\mbfvec}[1]{{\underrightarrow{\mbf{#1}}}}
\newcommand{\mbfdel}[1]{{\delta{\mbf{#1}}}}
\newcommand{\mbfDel}[1]{{\delta{\mbf{#1}}}}
\newcommand{\mbfdot}[1]{{\dot{\mbf{#1}}}}
\newcommand{\mbfddot}[1]{{\ddot{\mbf{#1}}}}

% A coordinate frame definintion
% edit lestefan: added \protect to make command suitable for usage in captions.
\newcommand{\cframe}[1]{{\smash{\protect\underrightarrow{\mathcal{F}}_{#1}}}}

%new notation for homogeneous coordinates:
\DeclareMathAlphabet{\mathbfit}{OML}{cmm}{b}{it}
\newcommand{\homo}[1]{{\mathbfit{#1}}}
\newcommand{\mbfhbar}[1]{{\overline{\homo{#1}}}}
\newcommand{\mbfhhat}[1]{{\hat{\homo{#1}}}}
\newcommand{\mbfhtilde}[1]{{\tilde{\homo{#1}}}}
\newcommand{\mbfhdel}[1]{{\delta{\homo{#1}}}}
\newcommand{\mbfhdot}[1]{{\dot{\homo{#1}}}}
\newcommand{\mbfhddot}[1]{{\ddot{\homo{#1}}}}
\newcommand{\mbfh}[1]{{\homo{#1}}}

% Vectors
%\newcommand{\Vec}[1]{{\underrightarrow{#1}}}

% Operators
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

% Quaternions
\newcommand{\qc}[1]{\left[{#1}\right]^+}
\newcommand{\qo}[1]{\left[{#1}\right]^\oplus}
\newcommand{\qi}[1]{{#1}^{\scalebox{0.5}{$-1$}}}
\def\ep{\epsilon}
\def\la{\lambda}

% crossmx
\newcommand{\crossmx}[1]{\left[{#1}\right]^\times}

% translation with vectors
\newcommand{\trans}[3]{\leftidx{_{#1}}{\mbf t}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity

% physical entities attached to and relating to coordinate frames
\newcommand{\pos}[2]{\leftidx{_{#1}}{ \mbf r}{_{#2}}} % position
\newcommand{\postilde}[2]{\leftidx{_{#1}}{\mbftilde r}{_{#2}}} % position
\newcommand{\posbar}[2]{\leftidx{_{#1}}{\mbfbar r}{_{#2}}} % position
\newcommand{\poshat}[2]{\leftidx{_{#1}}{\mbfhat r}{_{#2}}} % position
\newcommand{\posh}[2]{\leftidx{_{#1}}{\mbfh r}{_{#2}}} % position in homogeneous representation
\newcommand{\poshtilde}[2]{\leftidx{_{#1}}{\mbfhtilde r}{_{#2}}} % position in homogeneous representation
\newcommand{\poshbar}[2]{\leftidx{_{#1}}{\mbfhbar r}{_{#2}}} % position in homogeneous representation
\newcommand{\poshhat}[2]{\leftidx{_{#1}}{\mbfhhaz r}{_{#2}}} % position in homogeneous representation
\newcommand{\posdot}[2]{\leftidx{_{#1}}{\mbfdot r}{_{#2}}} % position

\newcommand{\lm}[1]{\leftidx{_{#1}}{\mbf l}{}} % landmark
\newcommand{\lmbar}[1]{\leftidx{_{#1}}{\mbfbar l}{}} % landmark
\newcommand{\lmhat}[1]{\leftidx{_{#1}}{\mbfhat l}{}} % landmark
\newcommand{\lmh}[1]{\leftidx{_{#1}}{\mbfh l}{}} % landmark in homogeneous representation
\newcommand{\lmhbar}[1]{\leftidx{_{#1}}{\mbfhbar l}{}} % landmark in homogeneous representation
\newcommand{\lmhhat}[1]{\leftidx{_{#1}}{\mbfhhaz l}{}} % landmark in homogeneous representation

\newcommand{\vel}[3]{\leftidx{_{#1}}{\mbf v}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity
\newcommand{\veltilde}[3]{\leftidx{_{#1}}{\mbftilde v}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity
\newcommand{\velbar}[3]{\leftidx{_{#1}}{\mbfbar v}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity
\newcommand{\velhat}[3]{\leftidx{_{#1}}{\mbfhat v}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity
\newcommand{\veldot}[3]{\leftidx{_{#1}}{\mbfdot v}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % velocity

\newcommand{\wind}[1]{\leftidx{_{#1}}{\mbf d}} % velocity
\newcommand{\windtilde}[1]{\leftidx{_{#1}}{\mbftilde d}} % velocity
\newcommand{\windbar}[1]{\leftidx{_{#1}}{\mbfbar d}} % velocity
\newcommand{\windhat}[1]{\leftidx{_{#1}}{\mbfhat d}} % velocity
\newcommand{\winddot}[1]{\leftidx{_{#1}}{\mbfdot d}} % velocity

\newcommand{\myvec}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbf #1}{}} % vector
\newcommand{\myvectilde}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbftilde #1}{}} % vector
\newcommand{\myvecbar}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbfbar #1}{}} % vector
\newcommand{\myvechat}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbfhat #1}{}} % vector
\newcommand{\myvecdot}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbfdot #1}{}} % vector
\newcommand{\myvecs}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbs #1}{}} % vector
\newcommand{\myvecstilde}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbstilde #1}{}} % vector
\newcommand{\myvecsbar}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbsbar #1}{}} % vector
\newcommand{\myvecshat}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbshat #1}{}} % vector
\newcommand{\myvecsdot}[2]{\leftidx{_{#2}\hspace{-1pt}}{\mbsdot #1}{}} % vector

\newcommand{\acc}[3]{\leftidx{_{#1}}{\mbf a}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % acceleration
\newcommand{\acctilde}[3]{\leftidx{_{#1}}{\mbftilde a}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % acceleration
\newcommand{\accbar}[3]{\leftidx{_{#1}}{\mbfbar a}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % acceleration

\newcommand{\rotvel}[3]{\leftidx{_{#1}}{\mbs \omega}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % rotational velocity
\newcommand{\rotveltilde}[3]{\leftidx{_{#1}}{\mbstilde \omega}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % rotational velocity
\newcommand{\rotvelbar}[3]{\leftidx{_{#1}}{\mbsbar \omega}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % rotational velocity
\newcommand{\rotvelhat}[3]{\leftidx{_{#1}}{\mbshat \omega}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % rotational velocity
\newcommand{\rotveldot}[3]{\leftidx{_{#1}}{\mbsdot \omega}{\IfValueTF{#2}{_{#2#3\hspace{2pt}}}{}}} % rotational velocity derivative

\newcommand{\C}[2]{\leftidx{}{\mbf C}{_{#1#2\hspace{2pt}}}} % rotation matrix
\newcommand{\Ctilde}[2]{\leftidx{}{\mbftilde C}{_{#1#2\hspace{2pt}}}} % rotation matrix
\newcommand{\Cdot}[2]{\leftidx{}{\mbfdot C}{_{#1#2\hspace{2pt}}}} % rotation matrix time derivative
\newcommand{\Cbar}[2]{\leftidx{}{\mbfbar C}{_{#1#2\hspace{2pt}}}} % rotation matrix
\newcommand{\T}[2]{\leftidx{}{\mbfh T}{_{#1#2\hspace{2pt}}}} % homogeneous transformation matrix
\newcommand{\Ttilde}[2]{\leftidx{}{\mbfhtilde T}{_{#1#2\hspace{2pt}}}} % homogeneous transformation matrix
\newcommand{\Tbar}[2]{\leftidx{}{\mbfhbar T}{_{#1#2\hspace{2pt}}}} % homogeneous transformation matrix
\newcommand{\q}[2]{\leftidx{}{\mbf q}{_{#1#2\hspace{2pt}}}} % quaternion of rotation
\newcommand{\qtilde}[2]{\leftidx{}{\mbfbar q}{_{#1#2\hspace{2pt}}}} % quaternion of rotation
\newcommand{\qbar}[2]{\leftidx{}{\mbfbar q}{_{#1#2\hspace{2pt}}}} % quaternion of rotation
\newcommand{\qhat}[2]{\leftidx{}{\mbfhat q}{_{#1#2\hspace{2pt}}}} % quaternion of rotation
\newcommand{\qdot}[2]{\leftidx{}{\mbfdot q}{_{#1#2\hspace{2pt}}}} % quaternion of rotation

\newenvironment{notation}{\vspace{3mm}\begin{tabular}[t]{r
			@{\;\;\;:\;\;\;} p{\hsize}}}{\end{tabular}\vspace{3mm}}
\newcommand{\nitem}[2]{\raggedleft $\displaystyle {#1}$ & #2\\}

\newcommand{\sinc}{{\mathrm{sinc}}}

\newcommand{\renderImage}[2]{\leftidx{_{#1}}{ \mbf I}{_{#2}}} % Image
\newcommand{\generalTwo}[2]{{\mbf #1}{_{#2}}} % general two 1_2
\newcommand{\generalThree}[3]{\leftidx{_{#1}}{\mbf #2}{_{#3}}} % general three blank
\newcommand{\pixel}[1]{{\mbfh u}{_{#1}}} % pixel coordinate
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argax}{arg\,max}
